Preventive Model-based Verification and Repairing for SDN Requests

Software Defined Networking (SDN) is a novel network management technology, which currently attracts a lot of attention due to the provided capabilities. Recently, different works have been devoted to testing / verifying the (correct) configurations of SDN data planes. In general, SDN forwarding devices (e.g., switches) route (steer) traffic according to the configured flow rules; the latter identifies the set of virtual paths implemented in the data plane. In this paper, we propose a novel preventive approach for verifying that no misconfigurations (e.g., infinite loops), can occur given the requested set of paths. We discuss why such verification is essential, namely, how, when synthesizing a set of data paths, other not requested and undesired data paths (including loops) may be unintentionally configured. Furthermore, we show that for some cases the requested set of paths cannot be implemented without adding such undesired behavior, i.e., only a superset of the requested set can be implemented. Correspondingly, we present a verification technique for detecting such issues of potential misconfigurations and estimate the complexity of the proposed method; its polynomial complexity highlights the applicability of the obtained results. Finally, we propose a technique for debugging and repairing a set of paths in such a way that the corrected set does not induce undesired paths into the data plane, if the latter is possible.

==> highlights.tex <==
\section*{Highlights}
\begin{itemize}
    \item Unavoidable misconfigurations can occur in Software Defined Networking%71
    \item Some sets of data paths cannot be configured without introducing additional paths%82
    \item We establish conditions for a precise implementation of a set of data paths%76
    \item A method for checking a precise implementation of a set of data paths is proposed%82
\end{itemize}
